Safe CoR: A Dual-Expert Approach to Integrating Imitation Learning and Safe Reinforcement Learning Using Constraint Rewards

In the realm of autonomous agents, ensuring safety and reliability in complex and dynamic environments remains a paramount challenge. Safe reinforcement learning addresses these concerns by introducing safety constraints, but still faces challenges in navigating intricate environments such as complex driving situations. To overcome these challenges, we present the safe constraint reward (Safe CoR) framework, a novel method that utilizes two types of expert demonstrations$\unicode{x2013}$reward expert demonstrations focusing on performance optimization and safe expert demonstrations prioritizing safety. By exploiting a constraint reward (CoR), our framework guides the agent to balance performance goals of reward sum with safety constraints. We test the proposed framework in diverse environments, including the safety gym, metadrive, and the real$\unicode{x2013}$world Jackal platform. Our proposed framework enhances the performance of algorithms by $39\%$ and reduces constraint violations by $88\%$ on the real-world Jackal platform, demonstrating the framework's efficacy. Through this innovative approach, we expect significant advancements in real-world performance, leading to transformative effects in the realm of safe and reliable autonomous agents.

==> README <==
              +---------------------------------------+
              |          THE IEEECONF CLASS           |
              | By Scott Pakin, scott+iecnf@pakin.org |
              +---------------------------------------+

Description
===========

The IEEEconf class implements the formatting dictated by the IEEE
Computer Society Press for conference proceedings
(ftp://pubftp.computer.org/press/outgoing/proceedings/instruct8.5x11.pdf).
IEEEconf.cls replaces latex8.sty and is compatible with any BibTeX
style, not just latex8.bst.  The goal was to produce a more faithful
implementation of the formatting rules and to do so with cleaner LaTeX
code than that provided by the latex8.* files.


Installation
============

Execute "latex IEEEconf.ins" to create IEEEconf.cls.  Install
IEEEconf.cls at an appropriate place in your directory tree (e.g., in
/usr/local/share/texmf/tex/latex/IEEEconf/ or
C:\localtexmf\tex\latex\IEEEconf\) and update the filename database,
if necessary.  See the UK TeX FAQ (http://www.tex.ac.uk/faq) for more
information on installing classes.

IEEEconf comes with prebuilt PDF documentation formatted for
U.S. Letter paper.  If you want to build the documentation from
scratch, the procedure is as follows:

    latex IEEEconf.dtx
    makeindex -s gind.ist IEEEconf
    makeindex -s gglo.ist IEEEconf.glo -o IEEEconf.gls
    latex IEEEconf.dtx


License
=======

Copyright (C) 2009 by Scott Pakin

This file may be distributed and/or modified under the conditions of
the LaTeX Project Public License, either version 1.3c of this license
or (at your option) any later version.  The latest version of this
license is in:

   http://www.latex-project.org/lppl.txt

and version 1.3c or later is part of all distributions of LaTeX
version 2006/05/20 or later.

